A Computational Framework for Modeling Emergence of Color Vision in the Human Brain

It is a mystery how the brain decodes color vision purely from the optic nerve signals it receives, with a core inferential challenge being how it disentangles internal perception with the correct color dimensionality from the unknown encoding properties of the eye. In this paper, we introduce a computational framework for modeling this emergence of human color vision by simulating both the eye and the cortex. Existing research often overlooks how the cortex develops color vision or represents color space internally, assuming that the color dimensionality is known a priori; however, we argue that the visual cortex has the capability and the challenge of inferring the color dimensionality purely from fluctuations in the optic nerve signals. To validate our theory, we introduce a simulation engine for biological eyes based on established vision science and generate optic nerve signals resulting from looking at natural images. Further, we propose a bio-plausible model of cortical learning based on self-supervised prediction of optic nerve signal fluctuations under natural eye motions. We show that this model naturally learns to generate color vision by disentangling retinal invariants from the sensory signals. When the retina contains N types of color photoreceptors, our simulation shows that N-dimensional color vision naturally emerges, verified through formal colorimetry. Using this framework, we also present the first simulation work that successfully boosts the color dimensionality, as observed in gene therapy on squirrel monkeys, and demonstrates the possibility of enhancing human color vision from 3D to 4D.

==> 00-00-todo.tex <==
Here is the record of modifications for April 11th.

\begin{enumerate}
    \item ...
\end{enumerate}


Here is a list of TODO items.
\begin{enumerate}
    \item 
\end{enumerate}

\newpage

==> 99-Code_of_Ethics.tex <==
\section{Code of Conduct}

We, the authors of this paper submission, affirm our commitment to upholding the ICLR Code of Conduct and adhering to the highest standards of integrity, inclusivity, and ethical research practices throughout the preparation and submission of this work.

\section{Code of Ethics}

We, the authors of this paper submission, confirm our adherence to the ICLR Code of Ethics, ensuring that our research is conducted responsibly, with integrity, and in alignment with ethical guidelines set forth by the conference.

==> Rebuttal/R01-Introduction.tex <==
\section{Introduction}

\blue{Figure 1 has been revised for clarity, emphasizing that the input to our eye simulation engine is strictly a hyperspectral image. Additionally, the descriptions for \CMFSim and \NScope have been renamed to avoid confusion.}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{assets/fig1_1116.pdf}
    \caption{Overview of our proposed framework for modeling the emergence of human color vision. Our simulation engine of biological eyes converts a scene stimulus \red{(hyperspectral image)} to a stream of optic nerve signals (Section 3\& Video~0:13). We simulate cortical learning purely from these optic nerve signals  (Section 4) and show the emergence of color vision. We show how to analyze the emergent neural color quantitatively with \red{Color Matching Function test Simulator (\CMFSim) and qualitatively with Neural Scope (\NScope)} (Section 5).}
    \label{fig:1}
\end{figure*}


==> Rebuttal/R02-Related_Work.tex <==
\section{Related Work}
\subsection{\red{Measurement of Color Dimensionality in Human Color Perception \blue{(new subsection)}}}
% \subsection{Complexity of Human Color Vision}
Color vision is a rich and complex system, with neural mechanisms, particularly within the parvocellular pathway (V1-V2-V4), playing a critical role in processing sensory inputs and transforming them into color perception—an ongoing area of research in neuroscience~\citep{livingstone1987psychophysical, zeki1978functional, li2014perceptual, liu2020hierarchical}. The characterization of human color space has a long history, from early 19th-century theories~\citep{young1802ii, von1867handbuch} to modern frameworks like CIELAB~\citep{CIE1976} and Color Appearance Models~\citep{fairchild2013color}, which account for phenomena such as nonlinear photoreceptor responses~\citep{krauskopf1992color} and adaptation to changing illuminants~\citep{von1902theoretische}. While these frameworks have advanced our understanding of color vision, the dimensionality of color remains a central focus in characterizing color experience. Although traditional theories linked color dimensionality directly to the number of cone types in the retina~\citep{young1802ii, von1867handbuch}, \cite{jacobs2018photopigments} demonstrated that this relationship is more nuanced, highlighting the complexity of how color dimensionality emerges. This work, therefore, shifts focus to the cortical system as a whole, exploring how the brain computationally processes sensory signals to achieve the color dimensionality characterized by~\cite{maxwell1856theory} and~\cite{grassmann1853theorie}, solely from sensory input.

==> Rebuttal/R03-Simulation_Engine.tex <==
% \section{Methods}

\section{Simulation Engine for Biological Eyes and Optic Nerve Signals}

We model the three primary functions of the human retina based on the known science.
The scene imagery is sampled from a dataset of hyperspectral images~\citep{arad2022ntire} (Fig.2.A). A model of fixational eye drifts~\citep{rucci2015unsteady,young2021emulated,martinez2013impact} generates a sequence of frames that sample different parts of the image. \red{The Mona Lisa video in Supplementary Video shows saccades for illustrative purposes, but in the learning simulation, we model only fixational drift.} Each frame is projected on the retina, stimulating a randomized array of cone cells, according to known cell density variation as a function of eccentricity (distance from the fovea)~\citep{curcio1990human} and known statistics of different cone cell types~\citep{carroll2000flicker} (Fig.2.B). Each cone cell converts the scene light into photoreceptor activations based on cone type spectral response functions~\citep{stockman_spectral_1999,stockman2000spectral} (Fig.2.C), followed by lateral inhibition from horizontal cells~\citep{wool2018nonselective,rodieck1965quantitative} (Fig.2.D). These signals are transformed into spike trains (Fig.2.E), then bundled into optic nerve signals (ONS), resulting in spatial distortion (Fig.2.F), turning a color scene stimulus into a noisy, spatially distorted ONS. Additional details are in Appendix A and Video 1:15.

One observation to make is that there are three invariant properties of the simulated retina (i.e. retinal invariants): cell positions, cell types, and horizontal cell connections. These properties are held constant during generation of ONS for a particular eye, but we use the engine with different values for these properties to generate ONS datasets for a diverse set of eyes. For example, we create datasets with different cone types, including monochromatic (L, M, S), dichromatic (LM, LS, MS), trichromatic (LMS) and tetrachromatic (LMSQ) configurations (Fig.2.4). The generated ONS becomes spatially noisier as the number of cone types increases, and we investigate how the cortex infers the inherent color dimensionality of these eyes purely from the encoded differences in their respective ONS. We will release the dataset and code for generating ONS upon acceptance.


==> Rebuttal/R05-Representation.tex <==
\section{Neural Representation of Color Space and \red{Analysis of Emergent Color Dimensionality} \blue{(renamed for clarity)}}

\setcounter{figure}{3}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{assets/fig4_1116.pdf}
    \caption{\blue{(Revised figure and caption)} Overview of our measurement methods of emergent color dimensionality, Color Matching Function Test Simulator (\CMFSim) \& Neural Scope (\NScope). 1. The goal of \CMFSim is to find the minimum number of primary colors that can be matched to any target colors. A match color is a weighted sum of primary colors, and coefficients are iteratively updated to minimize the perceptual error until convergence. 2. \NScope is a visualization tool for visual percepts, independent from the cortical learning loop. It is parameterized as a learnable $N\times 3$ matrix, and optimized to minimize the projection error to the target RGB image. 3. Example output of \CMFSim for the cortical model trained with trichromat retina after convergence. The matching errors for all target spectral light, ranging from 400nm to 700nm, first converge to zero error with 3 primaries, formally indicating that the model has 3D color vision.}
    \label{fig:4}
\end{figure*}
% \subsection{Theoretical Definition of Human Visual Perception}\label{sec:method_representation_theory}

We model color in the cortex as a vector in high-dimensional space, \colorvectorspace. This decision represents our view that the brain has both the freedom and the challenge of somehow inferring the intrinsic color dimensionality of the visual signals it is receiving along the optic nerve. 
% We define the visual percept $\VisualPercept{t}$ as a high-dimensional vector \colorvectorspace in a color space, representing the cortical color at each pixel.
% 
Specifically, we define a cortical decoding function $\DecodeOperator$ that takes the optic nerve signal $\OpticNerveSignal{t}$ at time $t$ and transforms it into its internal visual percept $\VisualPercept{t}$ (Figure 3), such that:
\begin{equation}
    \VisualPercept{t} = \DecodeOperator(\OpticNerveSignal{t})
\end{equation}
where each pixel in $\VisualPercept{t}$ is a $N$-dimensional vector. Inside \colorvectorspace, we assume that cortical color space emerges as a $K$-dimensional manifold. To measure this intrinsic dimensionality $K$, we introduce two methods: formal, numerical \red{Color Matching Function test Simulator} (\CMFSim); and intuitive, visual \red{Neural Scope} (\NScope).


\red{
\CMFSim (Color Matching Function Test Simulator) is our tool to formally quantify the color dimensionality that has emerged in the $R^N$ color space of the cortical model (Fig.4.1). \CMFSim treats the retina model and cortical model as a black-box color observer.
Specifically, we limit ourselves to showing the model two patches of scene color at random, distinct locations on the retina to reflect the effect of real-world viewing conditions, obtaining only a scalar score as feedback to indicate the difference in color appearance (with zero representing a color match).}
This interface is intentionally limited and identical to color matching experiments with human subjects. Then, resting on the formal, technical bedrock for colorimetry established by \citet{maxwell1856theory} and \citet{grassmann1853theorie}, we exhaustively probe to determine the minimum number of color primaries needed to match any test color through linear combination (Figure 4.1 \& Appendix C). For example, Maxwell found that most humans require $3$ primaries and are formally trichromatic, but red-green colorblind persons require only $2$ primaries and are dichromatic. We model diverse color observers and measure the color dimensionality of their emergent vision.

% % \blue{(Re-written for clarity)} 
% \blue{(Revised paragraph for clarity)} \red{Building on this, we address the theoretical question of whether cortical inference is essential for color vision. To investigate, we compare two scenarios: (1) a control experiment baseline, where optic nerve signals are represented directly as internal percepts without cortical inference, and (2) a learning-based model, where cortical processing is involved in shaping color perception. We demonstrate that the control experiment baseline fails to pass standard color matching tests, as \CMFSim reveals the color dimensionality to be reduced to $1$-D for observers with $3$ cone types (Appendix D). In contrast, the learning-based model (Fig.5) successfully reconstructs full color dimensionality, highlighting the critical role of cortical inference in color perception.}

\blue{* The description of our control baseline experiment has been moved to the next section for clarity.}



\red{
\NScope (Neural-Scope) is our tool to qualitatively display the emergent colors in $R^N$ by projecting into RGB color space (Fig.4.2). 
\NScope is a learnable $N\times 3$ matrix maps the emergent cortical color manifold in $\mathbb{R}^N$ linearly to conventional RGB color, in order to enable visual inspection of the emergent color vision.  
For our hyperspectral dataset, we project the data in two ways: (1) using conventional color processing to convert the hyperspectral data to RGB via CIEXYZ~\citep{commission1931commission}, and (2) using the learned cortical model to map the hyperspectral data into an $R^N$ representation. \NScope is then determined as the least squares fit between the RGB result from the first method and the $R^N$ pixels from the second.
% These parameters are optimized through supervised learning to minimize the projection error between visual percept $V_t$ and the RGB-projected hyperspectral image. 
It is important to note that \NScope is independently optimized as a visualization parameter, totally separate from the main cortical loop, ensuring that the cortex only processes optic nerve signals without any direct exposure to RGB images. 
}
\NScope provides striking color visualizations and complementary intuition visually, which are fully consistent with formal \CMFSim results.
For example, \NScope allows us to compute and contrast the color palettes of the three different types of human dichromacy (Figure 5). 

In sum, we model cortical color as vectors in \colorvectorspace, allow color space to emerge naturally through the hypothesized learning mechanism, and measure the emergent color space's dimensionality quantitatively with \CMFSim and analyze it visually with \NScope. 




==> Rebuttal/R06-Results.tex <==




\section{Simulation Results - Emergence of Color Vision}\label{sec:result_emergence}

Figure 3.2 begins with a model of typical human retina containing L, M and S cones, and illustrates the time-varying behavior of the cortical model as it learns color vision. The visualized prediction error decreases as the training progresses, and the internal percept converges to $3$-D color vision both formally (\CMFSim) and visually (\NScope imagery), shown in Figure 3.3. Notably, the visual timeline highlights that the cortical model learns color vision one dimension at a time: achieving monochromacy at 700 learning steps, dichromacy at 1,200 steps, and converging to trichromacy after $10^6$ steps. 
% This trend is consistent with child behavioral psychology findings~\cite{brown1990development}, illustrating the theoretical possibility that immature color vision in human infants is partially caused by the cortical learning.
At convergence, the cortical model has accurately inferred all retinal properties: spectral identity of each cell, cell positions and lateral inhibition neighbor weights (Figure 3.4).
% 
% 
\red{The emergence of 3D color vision remained consistent across various conditions. We varied the ratio of L:M cone cells in the simulated retinal patch, testing 2:1 (original), 1:1 (variant 1), and 1:2 (variant 2). In all cases, the configurations converged to 3D color vision, indicating that the framework is adaptable to variations in cone distributions.}


% \blue{(The rest of the original text in Section 6.)}


The remainder of this section shows \CMFSim and \NScope results at convergence for a diversity of simulation scenarios. Figure 4.3 dissects the \CMFSim analysis for the case where the retina contains $3$ cone types. The graphs show color matching function results using optimal sets of color primaries from $0$ to $4$ primaries, along with the residual perceptual error as a function of wavelength. 
The area under the curve (AUC) for each error graph suggests that the error falls to near-zero only with at least 3 primaries -- this formally proves that the color dimensionality is $3$. %, 


Figure 5 presents results of the hypothesized cortical learning in a diversity of color observers where the retina contains different numbers of cone cell types. 
This shows that the model learns $K$-dimensional color vision when the retina contains $K$ cone types. That is, when the retina contains 1, 2, 3 or 4 cell types, the cortical model converges on mono, di, tri, or tetrachromat color vision, formally quantified with \CMFSim (further analysis of tetrachromat models in Appendix F). And qualitatively, we observe that the \NScope images are grayscale for $K=1$, colorblind with only shades of blue and yellow for $K=2$, and full color with all trichromatic hues only with $K=3$ (Figure 5.1). 
Use of \NScope is limited  to color dimensionality up to 3, and is to not applicable to $K=4$ case, but \CMFSim formally confirms that 4-dimensional color emerges there. 
All variants of retinas with two cone types (protanopia, deuteranopia and tritanopia), converge to 2D color vision. But more striking, \NScope reveals hue shifts among these models that are consistent with color vision deficiencies studies~\citep{brettel1997computerized} (yellow-blue hues for deuteranopia / protanopia~\citep{judd1948color,graham1959studies} and 
% \TODO{teal-orange} 
teal-pink hues for tritanopia~\citep{alpern1983trit}) (Figure 5.2).

\blue{(Moved from Section 5, revised.)}
\red{
% Building on this, we address the theoretical question of whether cortical inference is essential for color vision. To investigate, we compare two scenarios: (1) a control experiment baseline, where optic nerve signals are represented directly as internal percepts without cortical inference, and (2) a learning-based model, where cortical processing is involved in shaping color perception. We demonstrate that the control experiment baseline fails to pass standard color matching tests, as \CMFSim reveals the color dimensionality to be reduced to $1$-D for observers with $3$ cone types (Appendix D). In contrast, the learning-based model (Fig.5) successfully reconstructs full color dimensionality, highlighting the critical role of cortical inference in color perception.
As a control experiment comparison for Figure 5, we address the theoretical question of whether cortical inference is essential for color vision. To investigate this, we compare two scenarios: (1) a control experiment baseline, where optic nerve signals are directly represented as internal percepts without cortical inference, and (2) a learning-based model, where cortical processing shapes color perception. The control experiment baseline fails to pass standard color-matching tests, as \CMFSim demonstrates that the color dimensionality is reduced to $1$-D even for observers with $3$ cone types (Appendix D). In contrast, the learning-based model (Fig. 5) successfully reconstructs the full color dimensionality, underscoring the critical role of cortical inference in achieving accurate color perception.
}



\blue{Remaining text in Section 6.}

==> Rebuttal/RS-04-CMF-SIM.tex <==
\section{Color Matching Function Tests \& \CMFSim}\label{sec:supp-cmfsim}

In the classical color matching theory of~\cite{maxwell1856theory} and~\cite{grassmann1853theorie}, an observer compares a test color \SPD, $t$, and a set of $K$ primary color \SPDs, $p_i$ for $i=1,..., K$ and tunes real weights $\alpha_i$ for each primary until a color match is achieved. If a particular weight has a negative value, primary light of that magnitude is added to the test color $t$ rather than to the other primary colors.  Mathematically, a color match is achieved when the matching \SPD $\sum_{i=1}^K\mathrm\alpha_i^+ p_i$ and test \SPD $t+\sum_{i=1}^K(-\alpha_i)^+p_i$ appear identical. Here, $\alpha_i^+$ is defined as $\max(\alpha_i, 0)$.

We simulate such classical color matching by formulating the retina model plus learned cortical model as a black-box color observer in the colorimetric sense. That is, we take the test and matching \SPDs, \red{simulate the stimulation on different parts of the retina for test and match color patches}, apply the retina encoding model $\RetinaEncodingOperator$ and the learned cortical decoder $\DecodeOperator$ to each separately, and iteratively update the weights $\alpha_i$ until there is no further improvement in the computed perceptual difference $E=\|\DecodeOperator(\RetinaEncodingOperator(\sum_{i=1}^K\mathrm\alpha_i^+ p_i))-\DecodeOperator(\RetinaEncodingOperator(t+\sum_{i=1}^K(-\alpha_i)^+p_i))\|_2^2$. Note that the optimal $E$ will not be close to zero if the primaries cannot match test color $t$.


The color dimensionality of an observer is formally equal to the minimum number of primary colors required to match any test color. \CMFSim simulates thousands of color matches to rigorously compute this dimensionality for any given retina model plus cortical model.  In \CMFSim, we simulate classical color matching function (CMF) tests of exhaustively attempting to match test colors equal to each monochromatic wavelength (100 samples from 400 to 700 nm), with a linear combination of $K$ primary colors. For the primary colors, we use distinct, monochromatic \SPDs.  We start CMF tests with a single primary, and add primaries one-by-one until all test wavelengths in the CMF can be matched successfully. The pseudocode for \CMFSim is described in Algorithm 1.

For example, for our cortical model to be formally measured as trichromat, we must show that there do not exist any 1 or 2 primaries that can pass the CMF tests, and show 3 primaries that succeed. A brute-force approach would be to exhaustively test all possible sets of $K$ primaries; for efficiency, we instead perform stratified sampling  to randomly generate a large number (e.g.~500) distinct sets of primaries for each choice of $K$. We require that all of these possible primary sets fail, with the aggregate perceptual error across all wavelengths being greater than a threshold $\epsilon$, before incrementing the CMF tests to $N$+1 primaries. 





